The Southern Wide-Field Gamma-Ray Observatory (SWGO): A Next-Generation Ground-Based Survey Instrument for VHE Gamma-Ray Astronomy

We describe plans for the development of the Southern Wide-field Gamma-ray Observatory (SWGO), a next-generation instrument with sensitivity to the very-high-energy (VHE) band to be constructed in the Southern Hemisphere. SWGO will provide wide-field coverage of a large portion of the southern sky, effectively complementing current and future instruments in the global multi-messenger effort to understand extreme astrophysical phenomena throughout the universe. A detailed description of science topics addressed by SWGO is available in the science case white paper [1]. The development of SWGO will draw on extensive experience within the community in designing, constructing, and successfully operating wide-field instruments using observations of extensive air showers. The detector will consist of a compact inner array of particle detection units surrounded by a sparser outer array. A key advantage of the design of SWGO is that it can be constructed using current, already proven technology. We estimate a construction cost of 54M USD and a cost of 7.5M USD for 5 years of operation, with an anticipated US contribution of 20M USD ensuring that the US will be a driving force for the SWGO effort. The recently formed SWGO collaboration will conduct site selection and detector optimization studies prior to construction, with full operations foreseen to begin in 2026. Throughout this document, references to science white papers submitted to the Astro2020 Decadal Survey with particular relevance to the key science goals of SWGO, which include unveiling Galactic particle accelerators [2-10], exploring the dynamic universe [11-21], and probing physics beyond the Standard Model [22-25], are highlighted in red boldface.

==> babelbst.tex <==
%%
%% This is file `babelbst.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `bblbst')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from babelbst.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file merlin.mbs.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
%% Copyright 1994-2004 Patrick W Daly
 % ===============================================================
 % IMPORTANT NOTICE:
 % This bibliographic style (bst) file has been generated from one or
 % more master bibliographic style (mbs) files, listed above.
 %
 % This generated file can be redistributed and/or modified under the terms
 % of the LaTeX Project Public License Distributed from CTAN
 % archives in directory macros/latex/base/lppl.txt; either
 % version 1 of the License, or any later version.
 % ===============================================================
 % Name and version information of the main mbs file:
 % \ProvidesFile{merlin.mbs}[2004/02/09 4.13 (PWD, AO, DPC)]
 % This is babelbst.tex for English.
 % It should serve as a model for other languages.
 % Alternatively, store it under a different name (e.g. englbst.tex)
 % and then \input it with a command in babelbst.tex.
\def\bbland{und}                \def\bbletal{et~al.}
\def\bbleditors{Herausgeber}        \def\bbleds{Hg.}
\def\bbleditor{Herausgeber}          \def\bbled{Hg.}
\def\bbledby{herausgegeben von}
\def\bbledition{Auf\/lage}        \def\bbledn{Aufl.}
\def\bblvolume{Band}          \def\bblvol{Bd.}
\def\bblof{von}
\def\bblnumber{Nummer}          \def\bblno{Nr.}
\def\bblin{in}
\def\bblpages{Seiten}            \def\bblpp{S.}
\def\bblpage{Seite}              \def\bblp{S.}
\def\bbleidpp{Seiten}
\def\bblchapter{Kapitel}        \def\bblchap{Kap.}
\def\bbltechreport{Technischer Bericht}
\def\bbltechrep{Techn.\ Ber.}
\def\bblmthesis{Diplomarbeit}
\def\bblphdthesis{Dissertation}
\def\bblfirst{Erste}            \def\bblfirsto{1.}
\def\bblsecond{Zweite}          \def\bblsecondo{2.}
\def\bblthird{Dritte}            \def\bblthirdo{3.}
\def\bblfourth{Vierte}          \def\bblfourtho{4.}
\def\bblfifth{F\^^b{u}nfte}            \def\bblfiftho{5.}
\def\bblst{.}  \def\bblnd{.}  \def\bblrd{.}
\def\bblth{.}
\def\bbljan{Januar}  \def\bblfeb{Februar}  \def\bblmar{M\^^b{a}rz}
\def\bblapr{April}    \def\bblmay{Mai}       \def\bbljun{Juni}
\def\bbljul{Juli}     \def\bblaug{August}    \def\bblsep{September}
\def\bbloct{Oktober}  \def\bblnov{November}  \def\bbldec{Dezember}
\endinput
%%
%% End of file `babelbst.tex'.

